An investigation of the Online Payment and Banking System Apps in Bangladesh

Presently, Bangladesh is expending substantial efforts to digitize its national infrastructure, with a significant emphasis on achieving this goal through mobile applications that facilitate online payments and banking system advancements. Despite the lack of knowledge about the security level of these systems, they are currently in frequent use without much consideration. To observe whether they follow the minimum global set standards, we choose to conduct static and dynamic analysis of the applications using available open-source analyzers and open-source tools. This allows us to attempt to extract sensitive information, if possible, and determine whether the applications adhere to the standards of MASVS set by OWASP. We show how we analyzed 17 .apks and a SDK using open source scanner and discover security flaws to the applications, such as weaknesses related to data storage, vulnerable cryptographic elements, insecure network communications, and unsafe utilization of WebViews, detected by the scanner. These outputs demonstrate the need for extensive manual analysis of the application through source code review and dynamic analysis. We further implement reverse engineering and dynamic approach to verify the outputs and expose some applications do not comply with the standard method of network communication. Moreover, we attempt to verify the rest of the potential vulnerabilities in the next phase of our ongoing investigation.

==> core/aa.tex <==
\newpage
Looking into the permission table we get to see that almost all the applications require permissions related to the internet connectivity which makes sense due to the purpose of the applications, that is to interface the internet banking and online payment. However, things get a bit interesting from here. We get to see that some of the applications demand for permissions which are no longer required to be asked manually to perform two step authentication using OTP since Google has already designed an API for that specific purpose. So using permissions such as RECEIVE\_SMS \& READ\_SMS makes no point in such usecase. Hence, these permissions lie in the region of gray area since it raises the question of concern regarding the violation of privacy. From here the level of suspicion increases as some of the applications require the permissions WRITE\_CONTACTS \& READ\_CONTACTS. It is not logical and common to see payment utility applications to have any need to read and write contacts. In addition to this, it is also visible from the table that applications also require permissions including BLUETOOTH, , RECORD\_AUDIO \& WRITE\_SETTINGS. Banking and MFS applications must not have required such permissions in any scenario since none of the permissions have anything to do with what the applications perform. It is obvious that the more the applications require permissions, especially not necessary for the actions they are supposed to perform, the more susceptible they become to attacks.\\

==> core/application_permissions2.tex <==
\begin{table}[h]
    \centering
    % \small
    \begin{adjustwidth}{-2cm}{}
    \begin{adjustbox}{width=19cm}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
      \hline
        
        MANAGE\_ACCOUNTS &  & \cmark &  & \cmark &  &  & \cmark &  &  &  & \cmark &  & \cmark &  &  &  & \cmark\\
        
        \hline

        CHANGE\_WIFI\_MULTICAST\_STATE &  & \cmark &  & \cmark &  &  & \cmark &  &  &  & \cmark &  & \cmark &  &  &  & \cmark\\

        \hline

        USE\_CREDENTIALS &  & \cmark &  & \cmark &  &  & \cmark &  &  &  & \cmark &  & \cmark &  &  &  & \cmark\\

        \hline

        WRITE\_SYNC\_SETTINGS &  & \cmark & \cmark & \cmark &  &  & \cmark &  &  &  & \cmark &  & \cmark &  &  &  & \cmark\\

        \hline

        REQUEST\_INSTALL\_PACKAGES &  & \cmark & \cmark & \cmark &  &  & \cmark &  &  &  & \cmark &  & \cmark &  &  &  & \cmark\\

        \hline

        REQUEST\_DELETE\_PACKAGES &  & \cmark &  & \cmark &  &  & \cmark &  &  &  & \cmark &  & \cmark &  &  &  & \cmark\\

        \hline

        READ\_SYNC\_STATS &  & \cmark & & \cmark &  &  & \cmark &  &  &  & \cmark &  & \cmark &  &  &  & \cmark\\

        \hline

        AUTHENTICATE\_ACCOUNTS &  & \cmark &  & \cmark &  &  & \cmark &  &  &  & \cmark &  & \cmark &  &  &  & \cmark\\

        \hline

        READ\_SYNC\_SETTINGS &  & \cmark &  & \cmark &  &  & \cmark &  &  &  & \cmark &  & \cmark &  &  &  & \cmark\\

        \hline

        READ\_PHONE\_NUMBERS &  &  & \cmark &  &  &  &  &  &  &  &  &  &  &  &  &  &\\
        
        \hline 

        WRITE\_MEDIA\_IMAGES &  &  & \cmark &  &  &  &  &  &  &  &  &  &  &  &  &  &\\

        \hline

        ACCESS\_ADSERVICES\_ATTRIBUTION &  &  &  &  & \cmark & \cmark &  &  &  &  &  &  &  &  &  &  &\\

        \hline

        ACCESS\_ADSERVICES\_AD\_ID &  &  &  &  & \cmark & \cmark &  &  &  &  &  &  &  &  &  &  &\\

        \hline

        ACCESS\_ADSERVICES\_TOPICS &  &  &  &  &  & \cmark &  &  &  &  &  &  &  &  &  &  &\\

        \hline

        CONNECTIVITY\_ACTION &  &  &  &  &  &  &  & \cmark &  &  &  &  &  &  &  &  &\\

        \hline

        WRITE\_CONTACTS &  &  &  &  &  &  &  & \cmark &  & \cmark &  &  &  &  & \cmark &  &\\

        \hline

        BLUETOOTH &  &  &  &  &  &  &  &  & \cmark & \cmark &  &  &  &  &  &  &\\

        \hline

        BLUETOOTH\_CONNECT &  &  &  &  &  &  &  &  &  & \cmark &  &  &  &  &  &  &\\

        \hline

        READ\_MEDIA\_VIDEO &  &  &  &  &  &  &  &  & \cmark &  &  &  &  &  &  &  &\\

        \hline

        WRITE\_SETTINGS &  &  &  &  &  &  &  &  &  & \cmark &  &  &  &  &  &  &\\

        \hline

        READ\_MEDIA\_AUDIO &  &  &  &  &  &  &  &  &  & \cmark &  &  &  &  &  &  &\\

        \hline


        NFC &  &  &  &  &  &  &  &  &  & \cmark &  &  &  &  &  &  &\\

        \hline

        READ\_APP\_BADGE &  &  &  &  &  &  &  &  &  &  &  & \cmark &  &  &  &  &\\

        \hline

        RECEIVE\_SMS &  &  &  &  &  &  &  &  &  &  &  &  &  & \cmark &  &  &\\

        \hline

        READ\_SMS &  &  &  &  &  &  &  &  &  &  &  &  &  & \cmark &  &  &\\

        \hline

        REQUEST\_IGNORE\_BATTERY\_OPTIMIZATIONS &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \cmark &  &\\

        \hline

        ACCESS\_COARSE\_UPDATES &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \cmark &  &\\

        \hline

    \end{tabular}
    \end{adjustbox}
    \end{adjustwidth}
    
    \caption{Required permission by target applications}
    \label{tab:Required permission by target applications}
\end{table}

